A Decay Chain Spin Analysis for SUSY and UED at the LHC

In this thesis we concentrate on the determination of the spin of an intermediate particle by using a decay chain. In SUSY the gluino is especially interesting for searches at the LHC, since it is a Majorana fermion which can produce like-sign dileptons in the final state. In UED the like-sign dilepton signature could occur as well from the decay of a bosonic KK-gluon. As we will show, angular distributions of the outgoing b-jets in SUSY and UED differ due to the different coupling structures. The effect from the different boosts of gluino and heavy gluon is shown to be much smaller. The hadronic UED cross section for KK-gluon KK-quark collisions is calculated in leading order and compared to the gluino squark collision in SUSY. The analytically given partonic cross sections are compared at the threshold.

==> danksagung.tex <==
\chapter*{Danksagung}

Ganz besonders m\"ochte ich mich bei Dr.~habil.~Andr\'e H.~Hoang
f\"ur die hervorragende Betreuung meiner Arbeit bedanken. Er
hat mich an das interessante Thema schrittweise
herangef\"uhrt  und war jederzeit bereit, meine zahlreichen Fragen
zu beantworten.

Bei Prof.~Dr.~Gerhard Buchalla m\"ochte ich mich bedanken, dass er
es mir erm\"oglicht hat, die Diplomarbeit am Max-Planck-Institut f\"ur
Physik zu schreiben, indem er sich als Aufgabensteller zur
Verf\"ugung gestellt hat.
Prof.~Dr.~Otmar Biebel danke ich f\"ur seine
n\"utzlichen Hinweise und Anregungen.

F\"ur die vielen lehrreichen  Diskussionen m\"ochte ich mich
bei Cailin Farrell, Christoph Rei\ss er, Pedro Ruiz-Femen\'\i a und
Maximilian Stahlhofen bedanken.
Den Mitgliedern der Theoriegruppe des Werner-Heisenberg-Instituts
und insbesondere meinen B\"urokollegen 
Andreas Biffar, Florian Hahn-W\"ornle, Max Huber, Stefan Kallweit,
Josef Pradler, Felix Rust und Tobias Schl\"uter danke ich
f\"ur ihre Hilfsbereitschaft bei der L\"osung jeder Art von Problemen
und vor allem f\"ur die sch\"one gemeinsame Zeit.

Schlie\ss lich m\"ochte ich bei meinen Eltern f\"ur ihre
Unterst\"utzung w\"ahrend mei\-nes gesamten Studiums bedanken.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "thesis"
%%% End: 

